Event-Frame Fusion for Inter-Frame Segmentation via Event-Guided Motion

Autonomous navigation requires precise and efficient semantic segmentation, yet existing frame-based approaches remain limited by motion blur, glare, latency, and the low temporal resolution (20-30 FPS) of conventional cameras, which leads to information loss between frames. Event cameras have emerged as an alternative sensing modality, capturing intensity changes asynchronously with high temporal resolution, high dynamic range, and sparse outputs. However, event-based algorithms still fall short of frame-based ones in accuracy, as most segmentation methods are designed for dense frame data. To overcome these limitations, we propose a hybrid vision architecture that combines conventional frame-based and event-based cameras. The system integrates two complementary components: (1) a compact Spiking Neural Network (SNN) with 42k parameters for motion estimation, and (2) a lightweight event-driven SNN with 0.84M parameters for frame-based semantic segmentation, which interpolates motion between frames to refine segmentation results. By predicting inter-frame segmentations, the framework achieves segmentation rates of up to 500 Hz with an energy consumption below 1.87 mJ per inference, while maintaining real-time GPU execution at frequencies up to 200 Hz. Additionally, our approach compensates for information loss in frames affected by blur or overexposure, enabling more robust perception in challenging conditions.

==> sec/0_abstract.tex <==
\begin{abstract}
% Autonomous navigation requires precise and efficient semantic segmentation, yet existing frame-based methods struggle with inherent limitations in dynamic environments. Conventional cameras operating at 20–30 FPS suffer from motion blur and glare and their low temporal resolution introduces latency and information loss between frames. Although higher frame rates could address temporal resolution issues, this approach leads to higher bandwidth, computational costs and energy consumption, as it processes largely redundant pixel data without addressing blur or glare problems. To overcome these limitations, we propose a hybrid vision architecture combining conventional frame-based camera and an event-based sensor offering microsecond-scale temporal resolution. This design enables energy-efficient inter-frame segmentation while inherently resolving blur and dazzling effects. To achieve this, our system integrates two main components: (1) a compact spiking neural network for frame-based semantic segmentation and (2) a lightweight event-driven Spiking Neural Networks (SNNs) for motion estimation, which interpolates motion information between frames and refines segmentation results. Evaluated on the DSEC-Semantic and DDD17 datasets, the proposed approach delivers high-accuracy segmentation at up to 500 Hz, maintaining low latency and power consumption while enhancing robustness against intra-frame information loss.


Autonomous navigation requires precise and efficient semantic segmentation, yet existing frame-based approaches remain limited by motion blur, glare, latency, and the low temporal resolution (20–30 FPS) of conventional cameras, which leads to information loss between frames. Event cameras have emerged as an alternative sensing modality, capturing intensity changes asynchronously with high temporal resolution, high dynamic range, and sparse outputs. However, event-based algorithms still fall short of frame-based ones in accuracy, as most segmentation methods are designed for dense frame data. To overcome these limitations, we propose a hybrid vision architecture that combines conventional frame-based and event-based cameras. The system integrates two complementary components: (1) a compact Spiking Neural Network (SNN) with 40k parameters for frame-based semantic segmentation, and (2) a lightweight event-driven SNN with 0.84M parameters for motion estimation, which interpolates motion between frames to refine segmentation results. By predicting inter-frame segmentations, the framework achieves segmentation rates up to 500 Hz with energy consumption below 1.5 mJ, while running in real time on a GPU. Additionally, our approach compensates for information loss in frames affected by blur or overexposure, enabling more robust perception in challenging conditions.
\end{abstract}


